LocoVLM: Grounding Vision and Language for Adapting Versatile Legged Locomotion Policies

Recent advances in legged locomotion learning are still dominated by the utilization of geometric representations of the environment, limiting the robot's capability to respond to higher-level semantics such as human instructions. To address this limitation, we propose a novel approach that integrates high-level commonsense reasoning from foundation models into the process of legged locomotion adaptation. Specifically, our method utilizes a pre-trained large language model to synthesize an instruction-grounded skill database tailored for legged robots. A pre-trained vision-language model is employed to extract high-level environmental semantics and ground them within the skill database, enabling real-time skill advisories for the robot. To facilitate versatile skill control, we train a style-conditioned policy capable of generating diverse and robust locomotion skills with high fidelity to specified styles. To the best of our knowledge, this is the first work to demonstrate real-time adaptation of legged locomotion using high-level reasoning from environmental semantics and instructions with instruction-following accuracy of up to 87% without the need for online query to on-the-cloud foundation models.

==> v3/experiments/retrieval_commands/1a.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.5$\\ 
    $\phi=[0,0,0,0]$\\ 
    $v^\text{limit}_x=0.7$\end{tabular}

==> v3/experiments/retrieval_commands/1b.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.4$\\ 
    $\phi=[0.0,0.2,0.7,0.5]$\\ 
    $v^\text{limit}_x=1.5$\end{tabular}

==> v3/experiments/retrieval_commands/2a.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.5$\\ 
    $\phi=[0.0,0.5,0.5,0.0]$\\ 
    $v^\text{limit}_x=0.5$\end{tabular}

==> v3/experiments/retrieval_commands/2b.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.4$\\ 
    $\phi=[0.0,0.2,0.7,0.5]$\\ 
    $v^\text{limit}_x=1.5$\end{tabular}

==> v3/experiments/retrieval_commands/3a.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.6$\\ 
    $\phi=[0.0,0.5,0.5,0.0]$\\ 
    $v^\text{limit}_x=0.3$\end{tabular}

==> v3/experiments/retrieval_commands/3b.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.5$\\ 
    $\phi=[0.0,0.0,0.5,0.5]$\\ 
    $v^\text{limit}_x=0.8$\end{tabular}

==> v3/experiments/retrieval_commands/4a.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.6$\\ 
    $\phi=[0.0,0.5,0.5,0.0]$\\ 
    $v^\text{limit}_x=0.3$\end{tabular}

==> v3/experiments/retrieval_commands/4b.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.6$\\ 
    $\phi=[0.0,0.5,0.0,0.5]$\\ 
    $v^\text{limit}_x=0.2$\end{tabular}

==> v3/experiments/retrieval_commands/5a.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.7$\\ 
    $\phi=[0.0, 0.5, 0.5, 0.0]$\\ 
    $v^\text{limit}_x=0.4$\end{tabular}

==> v3/experiments/retrieval_commands/5b.tex <==
\begin{tabular}[c]{@{}l@{}}
    $T=0.7$\\ 
    $\phi=[0.0, 0.2, 0.7, 0.5]$\\ 
    $v^\text{limit}_x=1.5$\end{tabular}

==> v3/experiments/tables/gait_tracking_short.tex <==
\begin{table}
    % \vspace{-12pt}
    \centering
    \scriptsize
    \caption{Performance comparison between contact tracking with and without compliance. The mean and standard deviation of the traveled distances for $1,\!000$ rollouts are reported for each terrain. The shaded values indicate the best among the two methods.}
    \label{table:gait_tracking}

    \begin{tabular}{llccc}
        \hline
        \multicolumn{1}{c}{\multirow{2}{*}{Gait}} 
        &\multicolumn{1}{c}{\multirow{2}{*}{$\delta$}} 
        &\multicolumn{3}{c}{\textbf{Traveled distance}~$\textbf{(m)}\uparrow$} 
        \\ 
        
        &
        &\multicolumn{1}{c}{\textbf{Rough}} 
        &\multicolumn{1}{c}{\textbf{Discrete}}
        &\multicolumn{1}{c}{\textbf{Stairs}} \\
        \hline\hline

        \multicolumn{1}{c}{\multirow{2}{*}{Pronk}}  
        & $0$& $15.13\pm 3.61$ & $17.34\pm 6.41$ & $13.56\pm 2.53$  \\
        & $0.5$ & \colorbox{lightgray}{$15.59\pm 3.38$}  & \colorbox{lightgray}{$18.42\pm 6.29$}  & \colorbox{lightgray}{$14.06\pm 2.74$}  \\
        \hline
 
        \multicolumn{1}{c}{\multirow{2}{*}{Trot}}  
        & $0$& $16.72\pm 3.53$ & $16.62\pm 6.50$ & $14.92\pm 2.82$  \\
        & $0.5$ & \colorbox{lightgray}{$16.84\pm 3.72$}  & \colorbox{lightgray}{$18.29\pm 6.18$}  & \colorbox{lightgray}{$16.34\pm 2.41$}  \\
        \hline

        \multicolumn{1}{c}{\multirow{2}{*}{Pace}}  
        & $0$& \colorbox{lightgray}{$17.11\pm 3.51$} & $17.48\pm 5.89$ & $16.83\pm 2.35$   \\
        & $0.5$ & $16.31\pm 3.95$  & \colorbox{lightgray}{$19.49\pm 5.77$}  & \colorbox{lightgray}{$18.18\pm 2.49$}\\
        \hline

        \multicolumn{1}{c}{\multirow{2}{*}{Bound}}  
        & $0$& $14.57\pm 2.91$ & $14.53\pm 5.64$ & $14.17\pm 2.29$  \\
        & $0.5$ & \colorbox{lightgray}{$16.04\pm 3.57$}  & \colorbox{lightgray}{$17.43\pm 5.16$}  & \colorbox{lightgray}{$15.48\pm 2.92$} \\
        \hline

        \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rotary\\gallop\end{tabular}}}  
        & $0$& $16.67\pm 3.56$ & $16.71\pm 6.20$ & $16.40\pm 2.88$  \\
        & $0.5$ & \colorbox{lightgray}{$18.18\pm 3.91$}  & \colorbox{lightgray}{$18.61\pm 5.08$}  & \colorbox{lightgray}{$18.04\pm 2.10$}  \\
        \hline
    
    \end{tabular}
\end{table}



==> v3/experiments/tables/text_image_qualitative.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Qualitative evaluation of retrieval performance using raw texts and preprocessed texts as images.}
    \label{table:retrieval}
    % chage table font size
    \footnotesize
    \begin{center}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lm{0.18\linewidth}lm{0.18\linewidth}l}
    \hline

    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query}}} 
    &\multicolumn{2}{c}{\textbf{Raw text}}
    &\multicolumn{2}{c}{\textbf{Text as image}} 
    \\ 

    &\multicolumn{1}{c}{\textbf{Retrieved instruction}} 
    &\multicolumn{1}{c}{\textbf{Parameters}}
    &\multicolumn{1}{c}{\textbf{Retrieved instruction}} 
    &\multicolumn{1}{c}{\textbf{Parameters}}\\
    \hline\hline

    \lang{you are a horse} 
    & \lang{jumping like a frog} 
    &\input{\MainPath/experiments/retrieval_commands/1a.tex}
    &\lang{run beautifully like a horse} 
    &\input{\MainPath/experiments/retrieval_commands/1b.tex}
    \\ \hline

    \lang{what is a horse?} 
    & \lang{a large puddle is in front of you, avoid it} 
    &\input{\MainPath/experiments/retrieval_commands/2a.tex}
    &\lang{run beautifully like a horse} 
    &\input{\MainPath/experiments/retrieval_commands/2b.tex}
    \\ \hline

    \lang{there's a bird} 
    & \lang{shh! someone is sleeping move quietly}  
    &\input{\MainPath/experiments/retrieval_commands/3a.tex}
    &\lang{let's hop like a rabbit!} 
    &\input{\MainPath/experiments/retrieval_commands/3b.tex}
    \\ \hline

    \lang{catch the bird!} 
    & \lang{shh! someone is sleeping move quietly}  
    &\input{\MainPath/experiments/retrieval_commands/4a.tex}
    &\lang{crawl low to the ground like a lion stalking prey}
    &\input{\MainPath/experiments/retrieval_commands/4b.tex}
    \\ \hline

    \lang{run! there's a danger!} 
    & \lang{there's an icy patch! go carefully!}  
    &\input{\MainPath/experiments/retrieval_commands/5a.tex}
    &\lang{there's a predator behind you, move fast!} 
    &\input{\MainPath/experiments/retrieval_commands/5b.tex}
    \\ \hline
    
    \end{tabular}
    }
    \end{center}
\end{table*}

==> v3/limitations.tex <==
\section{Limitations}~\label{section:limitations}
Despite the promising results, \acro still poses several limitations that need to be addressed to improve its performance and applicability in real-world scenarios:
\begin{enumerate}
    \item \textbf{False interpretation.} Based on our evaluation in Section~\ref{section:results_retrieval}, \acro fails to interpret queries correctly in approximately $20.5\%$ of instructions. This issue arises because the VLM module was trained on a dataset significantly smaller than the one used to train the LLM that generates the database. One potential solution to this limitation is to directly utilize the generative capabilities of the LLM for image captioning. Specifically, for BLIP-2, the model's decoder is jointly trained with an LLM to generate image captions, indicating its potential to produce structured text descriptions comparable to LLM-generated instructions. To compare database instructions with caption texts, a more advanced sentence encoder, such as Sentence-BERT~\cite{reimers2019sentence}, could be utilized. However, computational costs must be carefully considered when deploying this solution in real-time systems.
    \item \textbf{Lack of text and image fusion.} The current implementation of \acro cannot simultaneously interpret text and image queries. This limitation limits the robot's ability to understand its surroundings through images while adhering to real-time task-level instructions from human operators. Future work could focus on integrating text and image modalities to enhance scene understanding and task execution.
\end{enumerate}

==> v3/locovlm_loco/preliminaries.tex <==
\paragraph{Preliminaries}
Our locomotion controller is built on deep reinforcement learning (RL) and is trained under a blind locomotion setting, where the robot lacks direct measurements of the surrounding terrain properties~\cite{kumar2021rma,lee2020learning,ji2022concurrent,nahrendra2023dreamwaq}. Using the method proposed by~\citet{nahrendra2023dreamwaq}, the controller predicts the robot's explicit and implicit states based on a sequence of past observations through implicit context adaptation. The policy generates actions in the form of target joint angles that modulate the robot's motion to follow a reference command velocity.

